Order-Preserving outer automorphisms of free and surface groups

We give a complete classification to when a finite group of outer automorphisms preserves a bi-order on a non-abelian free group and bi-orderable surface groups. We also give another new criterion for an outer automorphism of $F_n$ induced by action of an $n$-strand braid to preserve a bi-order on $F_n.$ Using the new criterion, we produce examples of order-preserving whose underlying permutation is a full cycle which answers in affirmative a question of Kin and Rolfsen.

==> Figures/nPuncturedDisk.tex <==
\begin{center}
\begin{tikzpicture}
    \draw[line width=0.25mm] (0,0) circle (2);
    \fill   (0,-2) circle[radius=2pt];
    \fill   (-1,0) circle[radius=1.5pt];
    \fill   (-0.75,0) circle[radius=1.5pt];
    \fill   (-0.5,0) circle[radius=1.5pt];
    \fill   (0.5,0) circle[radius=1.5pt];
    \fill   (0.75,0) circle[radius=1.5pt];
    \fill   (1,0) circle[radius=1.5pt];
\end{tikzpicture}    
\end{center}

